From Dense to Dynamic: Token-Difficulty Driven MoEfication of Pre-Trained LLMs

Training large language models (LLMs) for different inference constraints is computationally expensive, limiting control over efficiency-accuracy trade-offs. Moreover, once trained, these models typically process tokens uniformly, regardless of their complexity, leading to static and inflexible behavior. In this paper, we introduce a post-training optimization framework, DynaMoE, that adapts a pre-trained dense LLM to a token-difficulty-driven Mixture-of-Experts model with minimal fine-tuning cost. This adaptation makes the model dynamic, with sensitivity control to customize the balance between efficiency and accuracy. DynaMoE features a token-difficulty-aware router that predicts the difficulty of tokens and directs them to the appropriate sub-networks or experts, enabling larger experts to handle more complex tokens and smaller experts to process simpler ones. Our experiments demonstrate that DynaMoE can generate a range of adaptive model variants of the existing trained LLM with a single fine-tuning step, utilizing only $10B$ tokens, a minimal cost compared to the base model's training. Each variant offers distinct trade-offs between accuracy and performance. Compared to the baseline post-training optimization framework, Flextron, our method achieves similar aggregated accuracy across downstream tasks, despite using only $\frac{1}{9}\text{th}$ of their fine-tuning cost.

==> sections/router_table.tex <==

\begingroup
    \renewcommand{\arraystretch}{1.5}
    \begin{table*}[!t]
        \centering
        \resizebox{\textwidth}{!}{
            \begin{tabular}{c|c|c|c|c|c|c|c|c|c}
                \toprule
                \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{Overall Accuracy}} & \multicolumn{2}{c|}{ \textbf{Expert 1}} & \multicolumn{2}{c|}{ \textbf{Expert 2}} & \multicolumn{2}{c|}{ \textbf{Expert 3}} & \multicolumn{2}{c}{\textbf{Expert 4}} \\
                \cmidrule(lr){3-4}
                \cmidrule(lr){5-6}
                \cmidrule(lr){7-8}
                \cmidrule(lr){9-10}
                & & \textbf{Precision} & \textbf{Recall} & \textbf{Precision} & \textbf{Recall} & \textbf{Precision} & \textbf{Recall} & \textbf{Precision} & \textbf{Recall} \\ 
                \toprule
                $\mname$ $\theta=0.9$ &   93.78 & 97.17 &	96.23 &	88.56 &	86.00 &	87.5 &81.71 &95.5 &97.47 \\
                $\mname$ $\theta=0.8$ &   90.87 & 95.93 & 92.14 & 87.17 & 80.92 & 92.65 & 95.58 & 79.48 & 73.1 \\
                $\mname$ $\theta=0.7$ &   89.86 & 95.36 & 90.84 & 85.43 & 83.17 & 90.76 & 94.13 & 89.33 & 74.76 \\
                $\mname$ $\theta=0.5$ &  92.36 &  94.08 & 90.65 & 92.05 & 95.38 & 82.00 & 68.99 & 85.61 & 66.33 \\
                $\mname$ $\theta=0.3$ &  95.22 & 96.95 & 97.65 & 84.2 & 80.63 & 83.3 & 76.53 & 82.3 & 17.88 \\
                \bottomrule
            \end{tabular}
        }
        \vspace{0.1 in}
        \caption{Classification accuracy of the Token-Difficulty-Aware Router with regard to the predicted labels and the derived ground truth labels. These results are based on the routing predictions of all the tokens of $7$ downstream tasks, aggregated across all layers. High accuracy across all $\mname$ models highlights the effectiveness of the router in learning token difficulty.}
        \label{tab:router_acc}
    \end{table*}
\endgroup
